GrAALF:Supporting Graphical Analysis of Audit Logs for Forensics

System-level audit logs often play a critical role in computer forensics. They capture low-level interactions between programs and users in much detail, making them a rich source of insight and provenance on malicious user activity. However, using these logs to discover and understand malicious activities when a typical computer generates more than 2.5 million system events hourly is both compute and time-intensive. We introduce a graphical system called GrAALF for efficiently loading, storing, processing, querying, and displaying system events to support computer forensics. In comparison to other related systems such as AIQL [13] and SAQL [12], GrAALF offers the flexibility of multiple backend storage solutions, easy-to-use and intuitive querying of logs, and the ability to trace back longer sequences of system events in (near) real-time to help identify and isolate attacks. Equally important, both AIQL and SAQL are not available for public use, whereas GrAALF is open-source. GrAALF offers the choice of compactly storing the logs in main memory, in a relational database system, in a hybrid main memory-database system, and a graph-based database. We compare the responsiveness of each of these options, using multiple huge system-call log files. Next, in multiple real-world attack scenarios, we demonstrate the efficacy and usefulness of GrAALF in identifying the attack and discovering its provenance. Consequently, GrAALF offers a robust solution for analysis of audit logs to support computer forensics.

==> design-old.tex <==
\section{Design}

In this section, we describe the design and implementation of \sysname.

\subsection{System Architecture}
\label{sec:sys_arch}

Most of the tools being used today for system forensics fall into one of the following categories: 1) manual search tools, 2) Keyword, regular expression and statistics based search tools, and 3) autonomous search tools. in the first category users utilize tools like \textit{grep} to look for what they believe to be relevant in a large body of logs. Manual tools while very flexible are susceptible to human judgments, slow on tracking evidences and will more often than not create a lot of false positives. The second category how ever offers more flexibility, tools such as Elastic Search\cite{elastic}, Loggly\cite{loggly}, AIQL \cite{gao2018aiql} are great with looking into large bodies of logs and finding a time window or a resource that matches a certain criteria with flexible interfaces and great performance. The third category tools employ complex machine learning models that automatically search for patterns \cite{du2017deeplog,nguyen2018diot,brown2018recurrent} . While such tools show great performance figures, human experts can not use them as a search tool.

Tools like \cite{gao2018aiql,gao2018saql,loglens} provide the user with causal analysis capabilities, this ability is limited within one or two steps. This vastly limits the usability of these tools for forensics back tasks where back tracing an artifcat to it's root cause, or tracking the effects of a resource is desired. To solve these limitations, \sysname provides an interface for the user to trace effect and causal paths with infinite length throughout the forensics graph.


We have two main design goals, 1) We want the user to be able to query her data without manually re-constructing causalities. 2) We want our tool to be usable with a as much diverse setups possible, this will give the user the freedom to use the storage systems he is more familiar with as well as logging tools he prefers.
In addition we choose to address one more limitation of many system call logging systems which is their lack of finer grained units than \textit{thread}. This granularity level will create a considerable amount of false positives in a casualty analysis environment. To address this limitation we introduce an \textbf{Execution Unit} concept to our model, user can choose to provide this using tools like \cite{lee2013beep,ma2016protracer}; or to leave it empty so the tool will assume one default execution unit for each thread. Further more supplying the thread information is optional as well, if provided will be added to graph structure, otherwise one default thread will be assumed for all the activities of the process.


A high level overview of \sysname is shown in Fig.~\ref{fig:sys_arc}. Logs are generated by \textit{linux audit log}, \textit{sysdig} or any other logging system capable of exporting a formatted output.In our experiments, in order to enrich logs we have used \cite{lee2013beep} system, but our model does not require such tool to be used. Logs once created are transported to a main machine where \sysname is installed; \sysname will convert the input data into a graph representation which then is passed to the back end module of choice to permanent or temporary storage. In this work we implement connectors for Neo4J, Postgresql and Mysql; how ever implementing connectors to other backends is possible by a minimal effort.

\sysname is comprised of four main modules, all of which are interchangeable with  similar tools; 1) Logging, 2) Reader, 3) Storage and 4) Querying. These modules are explained in more detail in the following sections.  We have implemented \sysname in 7K lines of code written in Java.


\begin{figure}
\includegraphics{figs/overview-crop.pdf}
\caption{A high level overview of \sysname.}
\label{fig:sys_arc}
\end{figure}

\subsection{Graph Structure}
In \sysname graphs contain four main levels which we call layers in this literature. The main executor in our model is \textit{Process} this node is considered to be the highest granularity in \sysname. Each \textit{Process} will spawn one or more \textit{Thread(s)}, these threads, can then start multiple \textit{Execution Unit(s)}. Each \textit{ExeUnit} then runs a system call to make changes/access a file or socket or other types of system resources. These layers are shown in an example in Fig.~\ref{fig:sample_model}.

As per limitation of the log collection tools we assume we might not always see a system call that starts the execution of a process or a thread, thus to account for that we use parent process information in the logs as a source, if we do not already have an execution, we will mark that as the execution of the process by its parents.

each edge in the graph represents a system call. If there are multiple system calls that has happened between a node -typically an execution unit - and another resource -typically a file or a socket- this is going to be represented with multiple edges as shown in Fig.\ref{fig:sample_model}.


\begin{figure}
\includegraphics[width=1.0\columnwidth]{figs/sample_model.pdf}
\caption{Sample Hierarchy In \sysname Graph Model }
\label{fig:sample_model}
\end{figure}


In order to reduce storage cost as well as making the graph more readable we introduce 4 compression levels. level 0 will contain all the edges along with all their meta data. Level 1, will group the edges based on their source, destination and the command, in order to preserve action order this mode keeps all the time stamps at which the edge has been traversed. This will create a smaller graph at the expense of loosing the meta data on each edge including call arguments for all the edges. Level 2 will keep only the first and last time stamp at which the edge has been traversed, this will lead to more loss in details but will make updating of the graph possible with less effort if data is being stored in a backend storage. Level 3 only keeps the initial edge and discards any occurrence of such event later on, this graph will loose most of the ordering in events but still keeps the high level causal relationship between nodes. User is able to choose the compression level desired by supplying a command argument to the program. Also to more efficiently query the graph we have introduced two query modes of \textit{normal} and \textit{verbose}, in verbose mode, each event will be represented using a single unique edge, where the normal mode groups similar edges into one to make the resulting graph more readable. Furthermore methods such as \cite{lee2013loggc,ma2016protracer,xu2016highFidelity,hossain2018dependence} can also be used both as part of the graph creation module or as independent systems to further reduce the size of the forensics graph.



\subsection{Logging}

System Logging and provenance data collection has been studied in the literature extensively. Different approaches has been taken to tackle problems ranging from quality of collected logs to performance overhead introduced by the tools \cite{lee2013beep,pohly2012hifi,bates2015trustworthy,muniswamy2006provenance,sysdig}. \sysname does not rely on a certain type of logger to produce the logs, the minimal set of fields required to create the graph is mentioned below; any logger that is capable of providing such fields as a formatted output can be used as a log source with \sysname .

\begin{itemize}
    \item time stamp : this is the time at which the system call happened
    \item system call number : this shows the system call that happened
    \item process : this will show which process is emitting the system call
    \item file descriptor info : this will show the file descriptor which will also include network handle if applicable
\end{itemize}

Logs can be enriched by some other common fields, including but not limited to :

\begin{itemize}
    \item parent process information
    \item ancestor process information
    \item file descriptor detailed information
    \item process execution information, eg. the path and arguments it has started with
    \item system call arguments
    \item user information this shows the process is run as
    \item thread information
    \item execution unit information
\end{itemize}

In our experiments we have used two loggers to generate logs, Linux Audit Log and Sysdig, some of the logs are enriched with execution unit information using BEEP\cite{lee2013beep}.

\subsection{Reader}

Reader module is in charge of reading the input logs. In our tool source can be either from pipes into the process, input stream or an stored file. How ever it will require a minimal implementation to add new data sources to the system. Logs stored in a database can also be used as input to \sysname, this is more explained in the future sections.

\sysname has three implemented reading modules:

\begin{itemize}
    \item CSV reader , this module reads comma separated value format files, this is to be able to read in files from prepossessing systems.
    \item Audit Log Reader, this module reads and processes Linux Audit Log files. Linux Audit Log has minimal information in it's records by default, this module is designed to enrich the logs by adding information about the parent process and file descriptors.
    \item sysdig reader, this module uses a format that can be supplied to sysdig to collect rich logs. Sysdig logs come rich with meta information.
\end{itemize}

\subsubsection{CSV Reader}

This module reads in logs in from a coma separated format file -or stream-. This is particularly more useful when the input is coming from other tools due to the portability of the format. CSV files while not the most efficient in the storage are still among the most used formats. This module as input configuration accepts the fields and their order which are present in the file. This will help the module know to map which column in the CSV to what field in the internal object structure. Once read each record is divided into a line graph that represents the record based on the graph model explained in \ref{sec:sys_arch}; Resulting graph is then transferred to the storage module.

\subsubsection{Audit Log Reader}

This module is designed to read the Linux Audit Log format from either a file or an stream. Linux Audit Log output by default is a key value pair record format which lacks file descriptor details as well as process lineage information. This module maintains tables that are used to trace process and file descriptor numbers included in audit records to their names. These tables are populated when opening of a file or starting of a process system call is observed. A garbage collection flushes old information out of these tables to endure memory efficiency.
Audit Log reader module reads and enriches the records then  a line graph of each record is created from the information in the record which is then sent to the storage module.




\subsubsection{Sysdig Reader}

As explained in the logging section, sysdig has a rich log format which reduces the burden of findin basic meta data as in the default Linux Audit Log. \sysname has a dedicated input reader module that reads in logs from Sysdig. Sysdig provides the output formatting functionality which has been used to set the output fields being stored; those same fields and their order will be then used to recover system behaviour from those logs. Sysdig logs not only contain fine grained information about the file descriptors which otherwise will be impossible to get from traditional tools like Linux Audit Log, but it also provides information of the parent and ancestor processes which will make it easier to build the forensics graphs reducing the chance of missed processes when their initial execution has not been observed in the logging period. Log format for this module can be supplied by the user as a configuration parameter.

As in other reader modules, each record will be translated to a line graph following the \sysname layer convention and sent to storage module.

\subsection{Storage And Data Retrival Module}

Storage is important as it provides persistent to logs. While \sysname is designed for very fast in-memory querying; it is still bound by the memory space that the host machine can spare. While this feature is good for analyzing small to moderate log files in detail or relatively larger files in non-verbose mode, this still can not be used for large scale logs gathered from an enterprise over months or years.

\sysname uses storage systems to achieve two tasks, 1) to convert the input data into persistent information 2) to query those information to create the forensic graphs desired by the user.

Log storage is a very strategic decision made in any organization, in order to account for different preferences and applicatoins, we design \sysname to be compatible with a plethora of back end storage systems. This will give the user a freedom to choose what back-end they prefer to use, as more so than not, these stored logs will be utilized by other tools as well.

We divide back-end storage systems into two broad categories, \textit{tabular} and \textit{graph based}. For tabular format we mainly focus on \textit{postgresql} but \sysname also supports  \textit{mysql} data bases which can also be extended to \textit{Microsoft SQL Server} and \textit{Oracle} with minimal query adjustments.
Graph data bases are also represented by \textit{Neo4j} in \sysname. While traditional data stores mostly support SQL as their main querying language, the same concept is still missing in the newly emerged graph data stores\cite{cypherisgood,francis2018cypher}; thus introducing a new graph database as back end will require rewriting of some sections to adapt to the new structure.  Our current graph database implementation works based on Neo4j's Cypher\cite{cypher} query language.

All the data retrieved from the back-end storage or input will be encoded in a similar data structure model to be used with the user interface model; this also enables the tool to regard the data same regardless  of its origin.

\subsubsection{Graph Model}

Graph model will be mainly used in a graph database but it can also be implemented using two tables in a traditional relational data store, vertices and edges; where all the vertex information will be stored in the vertices table and edges will be stored in the edges table. This will cause a more compact storage in relational data store but will cause slight overheads in querying since the query module will then have to deal with joining those two tables. This how ever imposes an overhead in dealing with the logs as tabular format of records in a relational database will have information on multiple nodes of the graph, namely, the process, the final affected resource as well as optional thread and execution unit information. These information are also available as meta information in graph data base storage nodes and edges.

When an actual graph database is being used as a back-end, however, user input queries will map to far less number of queries issued against the database to fetch and reconstruct the same forensics graph, minimizing the round trip times as well as query complexities.

To store information in a back-end data store minimizing the memory used to keep them we turn each record read from input into a small graph with a maximum of 5 nodes and a maximum of 4 edges. These 5 nodes are :

\begin{itemize}
    \item Parent Process
    \item Process
    \item Thread
    \item Execution Unit
    \item File, Socket, Pipe, etc
\end{itemize}

and edges will represent the connection between these nodes. This structure is then passed to the graph database using a query that will first ensure resources do not exist and then will insert them, any preexisting node will be kept to preserve space and quaryability.
Edge insertion on the other hand depends on the compression configurations. If a level 0 -no compression- is selected, every edge is inserted in the database. How ever with higher compression levels, an edge is inserted and future occurrences of the same edge are considered updates that will change or add to the time stamps on the edge. A buffer is maintain of all the pending insertions in the system and it checks for repeated nodes or edges being added  to the graph.

 Also in order to support better performances, multiple back-end databases can be utilized, each with data for a particular time window. This will help getting around the performance degradation of databases as shown in evaluation.

\subsubsection{Relational Data Stores}

Most tools today work with relational  data as their main format. Also other works have shown incompetency of graph databases like Neo4j \cite{gao2018aiql} when it comes to storing large sums of log data and their query ability. Thus to best utilize traditional storage systems we also provide support for such systems.

In order to store data in a relational format we use one table with as many fields as in the internal record object. This opens room for direct storage and retrieval of those records on the other hand how ever this comes at storage cost. Also as we will show in  the evaluation sections, querying information from a relational data base for longer back tracking tasks is more time consuming compared to same trace in a graph database.

Each record passed to the storage module from the reader modules will turn into an insert query with all its fields which have values.

Currently \sysname relational data module supports postgresql and mysql database servers as a tabular back end.

\subsection{Query Execution}

Query execution is the most important module in \sysname. This module is in charge of translating user input queries into one or many queries that can fetch the data from back-end storage or the in memory graph.

Once user issues a query to \sysname's console, query execution engine receives the input query, after parsing the query it decides whether the query is a configuration query which will make changes to program settings or it is a query to fetch data from the forensics graph. Configuration queries will be sent to the configuration manager which is in charge of maintaining the parameters and configurations of the \sysname. Data fetch queries based on the selected back-end will be routed to their corresponding module.

This module works in its own thread to be independent of the inserter thread. This provides the user with the ability to query the data as it is being processed and inserted into the database back ends. Asynchronous querying merges the information fetched from the database into nodes already in the memory to ensure seamless integration and continuity of the queries.

As per differences in query languages and models, each back-end database will require its own query parser module. To compensate these differences in our back end storage there are three main query execution modules in \sysname.
\begin{itemize}
    \item  Memory based query module
    \item SQL based Query Module
    \item Neo4j Cypher based query module
\end{itemize}

\subsubsection{Memory based}

This is the primary querying module as other modules also use in memory graphs to process their final results, this will reduce graph construction efforts in other modules, also provides a single interface to other modules to be able to consume the data.

In memory graph module maintains 3 hash maps which are used to create indexes on nodes and edges, one map contains information in a nested map model which starts by node type and then is mapped by their identifier. Other map uses a combination of identifiers from vertices to identify edges between each two nodes. Last hash map maintains a title-name-based map of the vertices; this will help with resolving regular expression and title matching queries faster.

Select queries will start based on their criteria, eg. if user is looking for processes, search starts by navigating to the type hash map, finding processes and then move to looking for title matches. If no title is expressed in the query, all the nodes in that type will be considered. To lookup nodes based on their names how ever, search starts from the name hash maps by fining keys that match the criteria then processing their values.

Edge selection happens after nodes are selected. To find edges, we pick all combinations of two nodes and we go through each finding their corresponding edges from the edge map based on the combined  identifiers of the nodes; if this search yields any results those edges will be evaluated against edge criteria in the input query, eg. if user is asking for write system calls, edges returned should have write set as their system call. This helps efficiently find the desired nodes while maintaining a small overhead of nodes.

Back select queries start by a select query which finds the leaf nodes in the final graph, these nodes will be the nodes user wants to back trace from. Then a Breath First Search traversal happens on the forensics graph, finding back traces from those nodes. After the first layer all nodes will have only one parent as one file or socket might be accessed by many processes how ever a process can not be created by more than one process. This assumption makes back tracking significantly faster as there is no need to do redundant lookups and also a lot of the graph paths converge to processes like `initd` or remote access clients like `sshd`.

Forward select queries are designed to see the effects of one node as it expands over other nodes. Like back selects, forward selects also start with a selection of the main nodes in question using a select query. Once the initial nodes -root or roots- are found, a breath first search will be done on the nodes following them level by level.

Breath first search is chosen as a uniform search strategy in graph traversals for two main reasons 1) each record in a log input will contain information about multiple levels of the graph, thus a DFS has a higher chance of redundant queries. 2) as explained before, specially in back tracking the parents will be a line graph starting from the first of second layer after the initial nodes. While this could benefit both DFS and BFS we stay with BFS for the entire \sysname to keep the model the same.

Once the nodes are explored all the nodes will be listed and their connecting edges will be added to the final graph from the edges map in accordance with the edge filter criteria supplied.

To maintain final results of queries as a graph data structure as well as it's presentation, we leveraged JUNG \cite{o2005jung} which provides a light weight wrapper and user interface presentation for graphs and networks.

\subsubsection{SQL based Module}

Much like the memory based module, once the input query is parsed and configuration queries are handled by the parent module, sql module will look for seen nodes in the database. in order to find right fields to query, if process information is given as a criteria, process, parent process and ancestor processes fields are considered in the initial query and then are fetched. When criteria are provided for a socket or file, file descriptor fields are the main source of filtering in the query. \sysname by default stops running of a user query with no criteria, this is due to the fact that real life logs will flood the memory and the output is going to be partial, thus by nature it can not be accurate or trusted. In order to stop missed conceptions we stop the query before running it.

Select queries will stop at this stage, all nodes that has been discovered will be sent to the memory module to create the final filtered graph.

To handle back select queries are once seed nodes are discovered, a breath first search will happen on the database following the trace. As mentioned in the previous section as each record contains information about the file or socket as well as its process, parent process and the ancestor process each fetched record will create between one and 4 layers of depth in the final graph. For each new level in the graph a new query is created and executed, until there is no more layers in the graph to follow. While this requires many queries \sysname tries to minimize the number of queries by merging queries for different paths in each layer into one query minimizing the round trip times and transaction creation overheads.

Forward select queries are handled in a similar way to the back selects except the fact that in a forward select maximum output degree of nodes are not one. To handle forward queries, \sysname runs the initial query to find the seed nodes, then it will run a breath first search for children of the nodes.


\subsubsection{Graph Based Module}

This model is the simplest among the query modules described. A graph database will already have the data stored in a graph model, thus there is no need for tedious repeated queries. Graph based module acts as an intermediary and will translate the user query into Cypher queries. Cypher queries are sent to the Neo4J database and the returned records are formed as a graph which will be appended to the graph already in the memory. Most \sysname queries are translated into one optimized Cypher statement.

Internal mechanisms of the graph database are trusted to be optimal when back tracing paths of arbitrary lengths, thus no particular graph traversal  method is applied in their case.


==> eval_databases.tex <==
\subsection{Database Evaluation}

Choosing a good backend database is very important as it affects the usability of data stored as well as the speed at which querying happens. While each database system offers its features, some are common among many, e.g., indexing. While \sysname offers the freedom of choice among many database systems, in this section, we evaluate Neo4j and postgress as two representatives of different server types. We evaluate the servers on two main criteria, insertion speed and querying speed. In both cases, we keep the server configuration to its default to keep fairness in comparison. While this does not reflect the best performance for either of the engines, it is aimed at providing a reference for comparison. Also, our main focus is to provide backend independence, so we do not try to optimize any one data store but try to show how they differ for the forensics back and forward tracking tasks; other works have suggested methods for indexing and optimizing the data in different databases \cite{gao2018aiql,gao2018saql,holzschuher2013graphDBperformance} and other high performance databases exist in the literature than can be leveraged as well \cite{maass2017mosaic}.

To evaluate insertions, we run 1000 queries per transaction for each of the backend servers. To maintain the uniqueness of nodes in Neo4j, we add a matching part to the insert query, which will reduce the performance but not considerably. Postgress data is being inserted into a single table.

Querying speed is done using three main metrics 1) a query that yields no results and 2) a query that grows in resulting graph size as more records are inserted and 3) a query which has an almost constant number of nodes and edges. Each of these queries has run on a fixed interval, and results are reported. A comparison of the empty result set is shown in Fig.~\ref{fig:empty_resutls_performance}, which shows a steady, very slow increase in time. The second query performance shows a faster increase compared to the first instance, but the rate is still steady, and reported times can be considered trivial, Fig.~\ref{fig:forward_select_performance}. The third query is shown in the set with a rising number in the returned set is shown in Fig.~\ref{fig:growing_results_performance}.

Insertion speed seems to grow at a steady pace for Neo4j, while the same performance for postgres moves more steadily. However, the surprising fact is the growth in time variance as numbers grow with Neo4j. Fig.~\ref{fig:insertion_performance} shows these comparisons of the insertions speeds.

Overall comparison of the results shown above shows while Neo4j is slower in insertion, it shows more steady performance as the forensics graph expands. Also, not only Neo4j outperforms the postgres in querying, but it shows far less variance in performance than that of postgress's.

Both database servers in question provide tools to speed up the insertions; however, they require making assumptions that might not always hold, eg. Neo4j offers a tool called \textit{batch insert} while this drastically improves insertion speed, it bypasses multiple layers of validations and ignores the whole concept of transactions this could lead to inconsistencies in the final database. However, it opens room for hybrid approaches where each database system can be used in part it is best at. As an example a hybrid system where postgress is used for initial data collection due to its non-trivial performance difference, then on a scheduled job, data can be processed and pushed into a Neo4j database for further evaluation as Neo4j querying performance shows far better querying performances, especially where backtracking and causality analysis is involved.

Furthermore, as insertion can be done in an asynchronous fashion, we also show how the length of the insertion queue changes over time. Fig.~\ref{fig:insertion_queue_len} shows this change, it can be seen that the length of queue increases when Neo4j is used, this is due to the fact that once the size of the data stored in a Neo4j database increases, the insertion time also increases, and this causes the queue to become longer. This slow down is also shown in Fig.~\ref{fig:processing_speed}.


The amount of memory that is dedicated to each computer can be selected in \sysname. This gives the user the ability to decide how much information he wants to keep in memory. \sysname will keep records it inserts in the memory until a memory threshold -by default set to 90\%- of the dedicated memory is used, then it starts to remove old nodes until the memory usage falls below the threshold. Fig.~\ref{fig:memory} shows how much memory will be used to keep how many hours of most recent logs in the memory so the user can make a more informed decision. Variance shown in Fig.~\ref{fig:memory} comes from periodic garbage collections, which reduces the used memory considerably.

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figs/insert_performance_per10k.pdf}
\caption{Insertion speed comparison, Neo4j vs. Postgres. Postgress time has been multiplied by 100 in order to make the trend more visible}
\label{fig:insertion_performance}
\end{figure}





\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figs/forward_select_performance_per10K.pdf}
\caption{Semi constant results query speed comparison, Neo4j vs. Postgres }
\label{fig:forward_select_performance}
\end{figure}

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figs/queLength.pdf}
\caption{Length of insertion queue in different backend data bases}
\label{fig:insertion_queue_len}
\end{figure}

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figs/memory_usage.pdf}
\caption{Amount of memory used to keep a forensics graph in memory for a single host }
\label{fig:memory}
\end{figure}

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figs/processing_speed.pdf}
\caption{Compares how different configurations can handle data in \sysname for a single machine stream. }
\label{fig:processing_speed}
\end{figure}


==> reviews.tex <==
\begin{document}

SUBMISSION: 106
TITLE: GrAALF: Supporting Effective Cyber Forensics Investigations
AUTHORS: Omid Setayeshfar, Christian Adkins, Matthew Jones, Kyu Hyung Lee and Prashant Doshi

----------- Overall evaluation -----------
The paper presents GrAALF, a graphical database system for maintaining and utilizing system events to support computer forensics. GrAALF is designed to support a number of functionalities such as compressed in-memory storage, a traditional relational database system, and a graph database for storing the parsed audit logs. It is evaluated on an extensive system call audit log of a real-world attack and shows that it can scale linearly with the number of records processed.

Overall, the paper is well written and detailed. However, the research contribution of the paper is not convincing. It does not present a research problem the requires efforts for novel solutions. GrAALF looks like a product development effort that can be useful for the industry but is not suitable for a security research conference.


----------------------- REVIEW 2 ---------------------
SUBMISSION: 106
TITLE: GrAALF: Supporting Effective Cyber Forensics Investigations
AUTHORS: Omid Setayeshfar, Christian Adkins, Matthew Jones, Kyu Hyung Lee and Prashant Doshi

----------- Overall evaluation -----------
The paper discusses a graph-based storage and query system with the particular intent of aiding forensics.

I really like this paper, and in my opinion, it should be published. It is very well written and modest and clear about what the system is. The paper also expresses a research experience which is interesting for me to read; for example, reconciliation of various log sources. Of course, one can always say negative things. One may argue that the work lacks conceptual depth. But to me, this is made up by the usefulness of such a system. Another criticism I have regards the design of the query language. It is clear that is kind of a graph-based language that suggests graph traversals. However, it says nothing about the intended application domain, i.e., forensics. If forensics is indeed a "killer app" for this system, then one would have thought that a syntax that is motivated by forensics is designed and provided. The example in Section 6.2 suggests an "attack graph" kind of syntax. So perhaps that can be the motivation for this kind of syntax for queries, i.e., the work on att!
 ack graphs and their utility in forensics.

In any case, I like this paper, and in my opinion, it should be published.


----------------------- REVIEW 3 ---------------------
SUBMISSION: 106
TITLE: GrAALF: Supporting Effective Cyber Forensics Investigations
AUTHORS: Omid Setayeshfar, Christian Adkins, Matthew Jones, Kyu Hyung Lee and Prashant Doshi

----------- Overall evaluation -----------
This paper proposes a system-level log analysis solution that consists of log ingestion, log storage and query layers. The authors claims the proposed system allows users to choose either relational database or graph database for the log data storage and query.  However, it is not clear whether the users need to choose one DB over the other for the entire system or per certain log data (if so, how). It is also unclear how practical and realistic for users to decide which kind of DB should be used. While the paper discusses pros and cons of relational and graph DBs in terms of log data causality traverse query and log insertion, no discussion on how this is used to decide which DB should be chosen is given. I am also wondering if the system can use both DBs and stores log data without any user intervention in a way to take advantage of both DBs. The authors claims all incoming queries are analyzed at in-memory storage and outputs are generated by querying the databases as nec!
 essary. A further discussion on how this query management is done could be helpful for better understanding. Overall, the paper presents an interesting approach that allows causality analysis of system log data using both relational and graph databases though it ultimately asks users to decide which type of DB should be used.

\end{document}
